A Bayesian Cognition Approach to Improve Data Visualization

People naturally bring their prior beliefs to bear on how they interpret the new information, yet few formal models exist for accounting for the influence of users' prior beliefs in interactions with data presentations like visualizations. We demonstrate a Bayesian cognitive model for understanding how people interpret visualizations in light of prior beliefs and show how this model provides a guide for improving visualization evaluation. In a first study, we show how applying a Bayesian cognition model to a simple visualization scenario indicates that people's judgments are consistent with a hypothesis that they are doing approximate Bayesian inference. In a second study, we evaluate how sensitive our observations of Bayesian behavior are to different techniques for eliciting people subjective distributions, and to different datasets. We find that people don't behave consistently with Bayesian predictions for large sample size datasets, and this difference cannot be explained by elicitation technique. In a final study, we show how normative Bayesian inference can be used as an evaluation framework for visualizations, including of uncertainty.

==> 4_study2_backup0920.tex <==
\vspace{-2mm}
\section{Study 2: Elicitation Techniques}
% \jessica{notes} 
% Motivating question 2 - Prior results assume we get their prior accurately. Method assumes full prior at individual level. But prior work indicates possibility that indivs only possess samples (e.g., this hypothesis can also yield optimal behavior). If so, elicitation that assumes complete distributions at individual level may not accurately characterize people's beliefs. Interval method may work for a single sample (e.g, mode is determined by most salient sample) but is motivated by analytical reasons, not match to people's mental representations (it is best for fitting a beta distribution compared to other text based full distribution elicitation). Alternative elicitation methods could yield  more accurate indiv fits by better capturing person's mental representation 
%     \begin{itemize}
%         \item Experiment 2: Assumptions: A better prior elicitation will suggest that people are more Bayesian at individual level/ aggregate level
%         \item Repeat procedure from Exp 1 but add condition 1: Sample based elicitation. If people have samples in their head, then asking for samples should provide an accurate representation.  Pros: match encoding of visualization, if confidence is elicited too (perhaps optionally), allows for some samples to be more salient than others. 
%         \item To distinguish between impact of matching vis encoding and impact of sample elicitation, also include a text based sample condition (they give same number of samples - e.g proportions with optional confidence).
%         \item Add condition 2: Balls and bins: sample-based, but assuming that participant can reason in terms of full distribution created by (100) samples
%     \end{itemize} 
% \jessica{end notes}


% For Bayesian approach to produce informative findings about visualization interpretation, the prior beliefs that are modeled should represent reasonable depiction of users' true mental representations of uncertainty. 

% \yeaseul{As the results of Study 1 alludes that people can be sample-based Bayesian, we would like to do something about it. If there were a sample based Bayesian }

%If they are sample-based Bayesian, the individual's posteriors will not aligned with the 


Study 1 used an elicitation technique from the literature which was designed for fitting beta distributions to participants' responses using a numerical solution~\cite{fox1966}. While the technique has been shown to be less sensitive to noise from the elicitation process than other techniques~\cite{wu2008}, it is possible that the evidence for noisy or ``sample-based'' Bayesian inference that we observed was in part an artifact of the elicitation technique. For instance, by asking for a modal value, it is possible that the technique prompted people to consider only a single sample. We are also interested in evaluating how robust our result in Study 1 is to changes in the dataset that is presented. 


%it has not been rigorously evaluated against other techniques which might better represent participants' internal representations of uncertainty. In particular, the close match between the normative Bayesian solution and the aggregate participants' posterior observed in Study 1 is predicted by a \textit{sampling hypothesis} proposed by prior work in Bayesian cognition~\cite{vul2014}. 
%A sampling hypothesis proposes that  Bayesian-in-aggregate behavior results from each individual reasoning with only a few samples. It is possible under this hypothesis that individuals do not possess a mental representation of the entire distribution at all. 
%Evidence for the sampling hypothesis may mean that eliciting subjective probability distributions from individuals--such as a graphical interface for describing a full subjective probability distribution in terms of discrete outcomes, as is suggested by the literature~\cite{goldstein2014}--is not ideal for eliciting people's prior and posterior judgments about many common types of data. \yeaseul{break the sentence}\yeaseul{raises the question of why we didn't use this to begin with}

In a second pre-registered study\footnote{\url{http://aspredicted.org/blind.php?x=4bf9ci}}, we therefore evaluate four different elicitation techniques (including interval elicitation from Study 1) and introduce a new dataset. 
The elicitation techniques we evaluate vary in the degree to which they ask a participant to provide a full distribution versus a small set of samples. 
By manipulating both the nature of the uncertainty representation that is being elicited and the dataset, we aim to gain a better sense of how robust our observation of noisy Bayesian inference is.
%We are first interested in understanding how far the aggregate posterior that is produced through each technique is from the normative aggregate posterior. A close alignment at the aggregate level is predicted by prior work in Bayesian cognition. We also compare the elicitation techniques at the individual level to better understand how sensitive individuals' (higher) deviation from the normative posterior is to elicitation technique. 

% should be that shows that people are in aggregate Bayesian. Our results from Study 1 suggest that the assumptions made in recent work in Bayesian cognition, where ``optimal'' Bayesian behavior is presumed to hold at the aggregate level.  


%The assumption behind our use of the aggregate KLD is that an elicitation technique that is more faithful to people's internal representations of uncertainty should result in the most optimal 
%, which alludes to minimizing the noise in eliciting a person's internal representation of uncertainty. 

% \yeaseul{Based on prior work in Bayesian cognition and collective intelligence, a judgment made by people collectively often considered as an optimal~\cite{}. Given that, we should observe the same phenomenon in our study, unless there is some noise in the study procedure (e.g., eliciting personal beliefs).}

%Additionally, by purposely evaluating elicitation techniques , 

%By comparing sample-based elicitation techniques to elicitation techniques that assume each individual possesses a mental representation of an entire distribution, or combine aspects of samples and full distributions, we hope to indirectly assess the nature of people's internal representations of uncertainty relevant to data interpretation. Furthermore, we hope to understand \textbf{what are the constraints of different elicitation techniques} regarding different data properties (e.g., sample size)? 

% . Lastly, by having a large number of participants complete a Bayesian comprehension task, we hope to investigate in more depth \textbf{how individuals update their prior beliefs in the context of data comprehension}. \yeaseul{previous sentence reflected the fact that we reported the individual level analysis in the study1, but this time we go a bit deeper}




% We ask, How does the deviation from the Bayesian normative solution at the aggregate level differ as a result of different elicitation techniques? \jessica{reconsider this sentence later:} By comparing sample-based elicitation techniques to elicitation techniques that assume that each individual possesses a mental representation of an entire distribution or represent a hybrid between samples and full distributions, we hope to indirectly assess the nature of people's internal representations of uncertainty relevant to data interpretation. 

\vspace{-2mm}
\subsection{Developing Elicitation Techniques \& Conditions}
We are interested in comparing a set of elicitation interfaces that vary in the format they use to elicit participants' responses. We describe two sample-based methods that we designed as well as two elicitation techniques from the literature.
While our data interpretation task requires eliciting a beta distribution, we expect that the techniques we evaluate should generalize to other symmetric distributions.

\subsubsection{Sample-based Elicitation}
Evidence from research on reasoning with uncertainty (e.g., on classical Bayesian reasoning tasks~\cite{gigerenzer1995}) and uncertainty visualization indicates that people are often better at thinking about uncertainty when it is framed as frequency rather than probability.
One way to elicit uncertainty is through a technique that asks people to provide one sample at a time until they have exhausted their mental representation. 
Imagine a person who is asked to provide their expectations for the proportion of women in tech who experience mental issues often. Several possible proportions seem salient to them, including 20\% and 33\%. We devise a sample-based elicitation method that asks a person to articulate a small set of samples (e.g., 5) one at a time (Fig.~\ref{fig:s2_technique}(a)). 

Even if people find it easy to reason  in the form of samples, its reasonable to expect that they might perceive some samples as more likely. A sample-based elicitation technique would not prevent a person from providing the same sample multiple times, proportional to its expected probability (i.e., resampling with replacement). However, articulating the same sample multiple times can be tedious. For each sample a person provides, our technique asks for a corresponding judgment about the salience of the sample in the form of subjective confidence. Using this technique, the hypothetical person with two samples of 20\% and 33\% might provide 20\% as a first estimate with a higher confidence (e.g., 70 on a scale of 0 to 100), and 33\% as a second estimate with a lower confidence (e.g., 30). In practice, the confidence values do not need to sum to 100 as they can be normalized prior to using them to fit the responses to a distribution. 
 
 
 We created two versions of our sample-based elicitation technique. A \textbf{graphical sample-based elicitation interface} (Fig.~\ref{fig:s2_technique} (a))
 allows participants to provide a predicted value (i.e., sample) by clicking icons in an icon array, similar to the visual format that we use to present the data, except for the elicitation icon arrays, we use circles\footnote{While in practice, we suspect that whether each icon is a circle or person will not greatly influence the responses people provide, a circle is a better metaphor for our desire to have participants think in terms of \textit{parameter space}, rather than the \textit{data space}.}
 
%  We provide an icon array comprised of 100 circles for eliciting each sample proportion. 
%  We also created a \textbf{text sample-based elicitation interface} that allows participants to provide the same number of samples via text input.
%  By default, both interfaces prompt participants to provide five total proportion estimates plus a confidence value (between 0 to 100) for each. 
%  While we require five samples, both techniques allow for the possibility that participants may naturally find only one or two samples salient by eliciting confidence (i.e., a participant could provide confidence 0 for all samples past their first) and by preregistering analysis of Bayesian behavior with differing numbers of samples used to fit distributions.
% \jessica{ we need to be linking to pre-reg somewhere}

% As a participant provides their samples, each prior sample is appended to the bottom of the interface so that participants can review their samples and corresponding confidence values before submitting the response. 
 

\subsubsection{Graphical Distribution Elicitation} 
To conduct a Bayesian analysis in many domains (e.g., clinical trials, meteorology, etc.), analysts probe domain experts for uncertainty estimates, then use these to construct a prior distribution~\cite{o2006}. This approach generally assumes that people with domain knowledge possess a relatively complete mental representation of the uncertainty in a parameter. Graphical elicitation of a full subjective distribution has been proposed for use among lay people, such as to elicit preferred retirement outcomes~\cite{goldstein2008}. Recent research indicates a graphical interface that enables constructing 
a distribution via placing 100 hypothetical outcomes  (``balls'', or circles representing hypothetical outcomes) in multiple ranges (``bins'') allows people to articulate a distribution that they have been presented with more accurately than a method that asks for quantiles of the distribution~\cite{goldstein2014}.
We implemented a \textbf{graphical ``balls and bins'' elicitation interface} (Fig.~\ref{fig:s2_technique}(c)).
Participants are prompted to add exactly 100 balls in bins that span between 0\% to 100\% in increments of 5\% to express the distribution they have in mind.
Relative to the text and graphical sample-based techniques we developed, the graphical balls and bins interface encourages a person to reason more about their entire subjective probability distribution.  
% \jessica{could probably shorten above section}

\subsubsection{Sample + Partial Distribution Elicitation}
The interval technique we used in Study 1 is best considered a hybrid approach between approaches that emphasize small sets of samples and those that emphasize a full distribution (Fig.~\ref{fig:s2_technique}(b)). The mode that a participant provides can be thought of as the most salient sample in their priors. The subjective probability that a participant provides is analogous to the probability mass of a partial distribution. 

As in Study 1, participants are first prompted to provide a prediction ($m$). Participants are then asked to provide the subjective probability ($sp$) that the true proportion falls into the range calculated based on the mode value that they entered  ([$m - m*0.25, m + m*0.25$]).\footnote{We elicited two additional random ranges to understand the effect of eliciting multiple ranges. The detailed analysis is in the supplemental material.}

% We made several changes compared to Study 1 in implementing the sample + partial distribution approach for Study 2. \jessica{Do we need to report on multiple ranges? Was that pre-registered? We might be able to footnote the fact that we elicited 3 and put any analysis that matters in the supplemental material, so we can save a bunch of space} Participants are first prompted to provide a prediction ($m$) as in Study 1. Participants are then asked to provide the subjective probability ($sp$) that the true proportion falls into the range calculated based on the mode value that they entered  ([$m - m*0.25, m + m*0.25$]). In contrast to Study 1, our technique in Study 2 asks for two additional intervals 1) to understand the effect of eliciting multiple ranges and 2) to compare the effect of the eliciting the subjective probability of the range associated the mode versus other random ranges that are not associated the most salient value for participants. To assign two ranges for which to elicit the subjective probabilities, we created a list of ranges from 0\% to 100\% spaced by 10\% ([0\%-10\%, 10\%-20\% ... 90\%-100\%]). We chose two ranges randomly among the range that did not overlap with the range associated with the mode. 
\begin{figure}[htb]
 \centering
  \includegraphics[width=3.5in]{./figures/vis.png}
 \caption{The data presentations for Study 1 (a) and Study 2 (a, b). }
\vspace{-6mm}
\label{fig:vis}
\end{figure}


\subsection{Study Design}

\subsubsection{Dataset and Presentation:}
We reuse the same proportion dataset used in Study 1 (mental health outcomes among women in the tech industry) and the same icon array visualization. However, we are also interested in understanding how robust the different elicitation techniques are to changes in the nature of the observed data. Specifically, the sample size of the observed data directly influences how closely the normative posterior is expected to align with the data. Intuitively, as the sample size of the observed data increases, the impact of the prior distribution on the normative posterior is reduced. With a very large sample, the normative posterior will be virtually indistinguishable from the data even with a reasonably concentrated prior distribution (Fig.~\ref{fig:s2_samplesize}). \sout{Ideally an elicitation technique would perform well across both of these cases.}


\begin{figure}[htb]
 \centering
  \includegraphics[width=3.5in]{./figures/s2_samplesize.png}
 \caption{The normative posteriors vary by the sample size of the observed data. In this example, we use the same prior distribution and the same mode to generate the observed data.}
\vspace{-0.1in}
\label{fig:s2_samplesize}
\end{figure}


% \yeaseul{(Fig ref). (would be nice if we could reference a figure, like a small one showing two frames of density plots - same prior in both, but different sample size datasets, so different normative posteriors). }

% The first dataset depicted the results of a survey that measured attitudes towards mental health in the tech workplace (N=747). and the proportion variable we used is: ``the proportion of women in the tech industry who feel that mental health affects their work often.'' 
% \jessica{need a slightly more persuasive motivation - why do we want to observe results across sample size rather than visualization type, parameter type, etc. I would think about this as a sensitivity analysis we present after we've shown results on the data set from Study 1. I think we could have a subsection after results called Sensitivity Analyses where we describe the three other datasets we ran and the no-elicitation condition we ran. Could also include number of samples analysis. We will just need to be clear about what was pre-registered and what was not} \yeaseul{we decided to use two datasets, and frame two opposite setting datasets as the replication.}

Therefore, we chose one additional large sample dataset that had previously been visualized in the New York Times using icon-style visualizations~\cite{nytElderly}. 
This dataset depicts the results of a study of chronic health conditions among assisted living center residents in the U.S. (N=750,000). We chose one type of chronic health condition (Alzheimer's disease or another form of dementia) to formulate our target proportion. We asked participants to reason about ``the proportion of residents who have Alzheimer's disease or another form of dementia'' in the task. We created a visualization (Fig.~\ref{fig:vis} (b)) that shows this proportion in a similar icon array format to that used for the mental health in tech dataset. Because of the size of the sample, we tell participants that each icon represents 600 residents of assisted living center. 


\subsubsection{Procedure}
We used the same procedure as in Study 1 (eliciting priors, presenting observed data, eliciting posteriors). However, in Study 2 we randomly assigned participants to one of four elicitation conditions. On the last page of the experiment, we asked a pre-registered attention-check question about the numeric range in which the observed proportion fell to exclude participants who may not have paid attention to the observed data. Participants were asked to choose an answer among three ranges (0\%-30\%, 30\%-60\%, 60\%-100\%).

\subsubsection{Dependent Measures}
Methods used in previous research compare elicitation techniques by examining which leads to the most accurate response distribution after exposing participants to a reference distribution~\cite{goldstein2014, hullman2018}. However, minimizing deviation from the Bayesian normative posterior at an individual level may not be realistic if people are only approximately Bayesian individually ~\cite{vul2014}. We instead wish to know which elicitation technique most reduces the deviation between the aggregate posterior distribution and the normative Bayesian posterior. We use the same measure of distance between two distributions that we used in Study 1, namely KLD. 

In addition, we would like to analyze individuals' KLDs to understand how they are affected by elicitation techniques. Through this analysis, we can investigate the degree to which the optimal behaviors at aggregate level are an outcome of all individuals being more Bayesian, or extreme individual KLDs that cancel one another out.


\subsubsection{Participants}
Based on a prospective power analysis conducted on pilot data with a desired power of at least 0.8 assuming $\alpha$=0.05, we recruited 800 workers with an approval rating of 98\% or more (400 per dataset, 100 per condition) in the U.S from Amazon Mechanical Turk (AMT). We excluded participants who did not respond correctly to our attention check question from the result according to our pre-registration. We posted the task to AMT until 800 participants who correctly answered the attention check question were recruited. Participants received \$0.6 as a reward. 




\subsection{Results}
\subsubsection{Data Preliminaries}
\textbf{Task completion time:} The average time to complete the task was 4.8 minutes (SD=3.35). 

\textbf{Fitting Distributions to Participants' Responses}
For each technique, we aimed to use the most direct and simplest way of fitting a beta distribution, so as to minimize noise contributed by the fitting process. 
For sample-based elicitation conditions, we used the Method of Moments~\cite{hansen1982} to estimate distribution parameters (i.e., alpha and beta) using samples provided by each participant. This method provides an estimate using the mean of the samples that participants provided ($\bar{x}$) and the variance of the samples ($\bar{v}$) to calculate beta parameters: $\alpha = \bar{x}(\frac{\bar{x}(1-\bar{x})}{\bar{v}} -1), \beta = (1-\bar{x})(\frac{\bar{x}(1-\bar{x})}{\bar{v}} -1)$. Since we asked participants to provide their subjective confidence with each sample, we calculated weighted $\bar{x}$ by multiplying the value of each sample by the corresponding confidence value. This approach does not provide a unique solution when the participant provides the same values five times or 0 confidence for all samples. In this case, we gave the participant an uninformative uniform prior ($\alpha=1, \beta=1$). We provide a sensitivity analysis to different ways of interpreting these ``deviant''cases in the supplemental material. For full distribution condition, we also used the Method of Moments approach by considering each ball as a sample known within a 5\% (the bin width). 
For the sample \& partial distribution condition, we used the same optimization approach we used in Study 1 that found an optimal distribution parameterized by alpha and beta that best represents the participants' mode and the subjective probability of the given interval. 
 
 \begin{figure}[htb]
 \centering
  \includegraphics[width=3.5in]{./figures/s2_agg_avg_kld.png}
 \caption{ Density plots of KLDs at an individual and aggregate level by condition and dataset.}
\vspace{-0.1in}
\label{fig:s2_agg_avg_kld}
\end{figure}

\subsubsection{Comparison of Aggregate KLD}
Figure~\ref{fig:s2_agg_avg_kld} shows the aggregate KLD for each condition and two datasets along with bootstrapped 95\% confidence intervals. We randomly drew 100 samples from each condition with replacement, calculated the aggregated level KLD, repeated this process 2000 times and calculated the 95\% confidence interval of KLDs from 2000 times of bootstrapping (Fig.~\ref{fig:s2_agg_ci} (a))).

\begin{figure}[htb]
 \centering
  \includegraphics[width=3.5in]{./figures/s2_agg_ci.png}
 \caption{Bootstrapped 95\% confidence intervals for aggregate KLDs. (a) is the result of the original sample sizes of the datasets and (b) is the result from the replication. }
\vspace{-0.1in}
\label{fig:s2_agg_ci}
\end{figure}

In the tech dataset (N=158), the text sample-based condition (CI:[-2.76,-2.21]) and sample + partial distribution condition (CI:[-2.1,-1.95]) yielded smaller KLDs than the other two conditions. This result is followed by the graphical sample-based condition (CI:[-1.18,-0.64]) and the full distribution condition (CI:[-0.46,0.09]). In the elderly dataset (N=750,000), the graphical sample-based condition produced a smallest aggregate KLD (CI:[1.19,1.22]), followed by the text sample-based condition (CI:[1.26,1.28]). The full distribution condition produced a highly varied result between participants (CI:[1.28,1.44]). Unlike the tech datasets, the sample + partial distribution condition produced the largest log KLD (CI:[1.42,1.43]).

\textbf{Replication on Modified Datasets:}
To better understand the impact of sample size vs. the nature of what the data described, we re-ran the same study with the modified setup of the sample size; we presented the tech datasets as a large sample survey (N=720,000), and the elderly dataset as a small sample study (N=150). The results depicted similar patterns to those observed with those of the original setup (Fig.~\ref{fig:s2_agg_ci} (b))). In the elderly dataset (N=150), the text sample-based condition achieved the lowest aggregate log KLD (CI:[-2.66,-2.1]), followed by the sample + partial distribution condition (CI:[-1.42,-1.35]), the graphical sample-based condition (CI:[-0.73,-0.26]), and the full distribution condition (CI:[-0.03,0.33]). In the tech dataset (N=720,000), the graphical sample-based technique produced the lowest aggregate KLD (CI:[1.23,1.25]), followed by the text sample-based technique (CI:[1.31,1.32]), the full distribution condition  (CI:[1.34,1.35]) and the sample + partial distribution condition  (CI:[1.36,1.37]).

\setlength{\columnsep}{10pt}
\begin{wrapfigure}[11]{r}{0.27\textwidth} 
\vspace{-8pt}
  \begin{center}
    \includegraphics[width=0.27\textwidth]{figures/s2_sample_num.png}
   \end{center}
      \caption{The aggregate log KLDs based on how many elicited samples to construct participants' prior/posterior distributions.}
  \label{fig:s2_sample_num}
\end{wrapfigure} 
\ 

\textbf{Determining Optimal Number of Samples:} Per our pre-registered analysis plan, we also analyzed the effect of the number of samples. We used the first n-th samples (2 $<$ n $\leq$ 5) that participants provided to calculate aggregate log KLD. Figure~\ref{fig:s2_sample_num} shows the changes in the aggregate log KLDs based on the number of samples being used to represent each participants' beliefs. In the tech dataset (N=158), using first four samples produced the lowest aggregate log KLD. In the elderly dataset (N=750,000), however, using two samples yields the lowest result. 

\vspace{-3mm}
\subsubsection{Constraints of Each Technique:}
While the elicitation techniques we tested do not explain the difference in how Bayesian people appear to be for the small vs. large sample size datasets, we did observe some differences in people's response distributions that may arise from the elicitation technique.

%However, we observed some reliable differences for the small sample size data makes it worth reflecting on each technique's constraints.
% The sample + partial distribution technique produced the lower log KLD for a smaller sample size in datasets (Study 1 and Study 2). However, for expressing uncertainty as a highly concentrated distribution, the technique has inherent limitation. We used a pre-specified constant k (k=0.25) to generate the interval participants were prompted for ([$m - m*k, m + m*k$, k is pre-specified]). As the mode increases, participants lose an ability to express a highly concentrated distribution. For example, when a participant provides a mode of 0.5, the prompted interval will be [0.375, 0.625]. Even if the participant responded 100\% to the interval, the final distribution will be fairly smooth bell-curved. With limited discussion on the effect of varied $K$ in the literature, the technique remains limited in applications across datasets of varied sample sizes. 
For example participants in the graphical distribution condition tended to construct roughly symmetric distributions near the center of the interface. 
We counted the participants whose responses spanned more than three bins, with the number of balls on either side of the center differing by less than two balls. 110 out of 200 participants in this condition attempted to create a symmetric distribution across more than three bins (total 15\% range) for their posterior distribution. Also, we observed responses from 137 participants (out of 200) put the balls in the middle bins (i.e., 50\% ~ 55\%, 55\%~60\%).
Prior work on graphical elicitation has commented on the potential for people to be implicitly influenced by the axes ranges of an elicitation interface. In the case of the graphical distribution interface, it is possible that participants felt that their distribution should be roughly centered. 
%This observation may be able to account for a slightly better KLDs for the elderly dataset that has the mode as 42\% than the tech dataset (17\%). Together, these compulsions might contribute to the low performance of this condition. 

In deploying sample-based techniques, we did not force participants to provide different values for each prediction. 62 participants (out of 400 from the graphical and text sample-based conditions, 15.5\%) provided a single value for all five samples. We can interpret this response as if the participant did not carry any uncertainty information (i.e., uninformative uniform distribution), as we did in this study, or as a highly concentrated distribution (i.e., very peaked). In supplemental material we show how these interpretations impact our results.

%Somewhat surprisingly the graphical sample-based and text sample-based techniques did not perform similarly. For example, the graphical sample-based technique produced the lowest aggregate log KLD better on the larger sample size datasets than the smaller sample size datasets, while the text sample-based technique consistently yielded the lowers aggregate log KLD.

\begin{figure}[htb]
 \centering
  \includegraphics[width=3.5in]{./figures/s2_indi_ci.png}
 \caption{Bootstrapped 95\% confidence intervals for the individual average log KLDs.}
\vspace{-0.1in}
\label{fig:s2_indi_ci}
\end{figure}

\subsubsection{Comparison of Individual KLD}
\jessica{Start with individual - For small datasets, we see the same pattern (could be noisy Bayesian). For large, people are systematically overweighting their prior. - transition to replicated stuff - to disambiguate whether this  difference is due to the different domains of the data or the different samples size, we replicated. It appears to be sample size - transition to aggregate -- To confirm that we still see alignment with the normative posterior at the aggregate level for the small datasets, we assessed the aggregate level results. We find that while people's responses are still consistent with a noisy or sample-based Bayesian hypothesis for small datasets, we do not see analogous evidence that people's behavior is Bayesian for the large sample datasets.}
In all conditions, individuals' posteriors were closer to the Bayesian normative posteriors for the tech datasets than for the elderly datasets (Fig.~\ref{fig:s2_indi_ci}). We speculate that the deviation is caused by a well-documented tendency among people to show insensitivity to sample size and its relationship to variance (sampling error)~\cite{tversky1974}. Hence participants did not weight the observed data of the elderly dataset as much as they should, given the elderly dataset was from the large sample (N=750,000). 

One benefit of obtaining distributions rather than just expected values (e.g.,~\cite{kim2017, kim2018}) is that we can interpret the parameters of the fitted beta distributions to gain insight into how participants perceived the data. For a beta distribution, two parameters $\alpha$ and $\beta$ are associated  with the sample size that the distribution represents. $\alpha$ stands for the number of successful trials, and $\beta$ stands for the number of failed trials. By using the participants' posteriors as normative posteriors and the given priors, we reverse-calculated the perceived observed data distribution ($\alpha_\text{perceived data}$ and $\beta_\text{perceived data}$) for each participant, then summed these two parameters. 
Figure ~\ref{fig:s2_perceivedsample} shows how the perceived sample size of the observed data was roughly the same. The mean across all techniques for the tech dataset (N=158) was 212.47 (median=41.14) whereas the mean of elderly dataset (N=750,000) was 359.58 (median=51.51), despite the enormous actual difference in the sample sizes of the observed data (158 vs. 750,000). 

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=3.5in]{figures/s2_perceivedsample.png}
   \end{center}
   \vspace{-5pt}
      \caption{The perceived sample size analyzed by participants' prior and posterior distributions. The participants had similar perceived sample size between two very different datasets in terms of the sample size.}
    \label{fig:s2_perceivedsample}
    \vspace{-4mm}
\end{figure} 

\subsection{Summary of Results}
% At the aggregate level, the text sample-based technique produced the lowest log KLD. But we did not see much difference in individual-level log KLD. 
We again observed evidence that participants were Bayesian for our original dataset (N=152), as well as a second dataset of the same size. However, we did not see comparable evidence for Bayesian behavior for either large sample size dataset. While we observed some variance in results based on elicitation technique for the smaller datasets, elicitation technique was \textit{not} sufficient to explain the differences in results between the small and large sample size datasets. %, but sample size affected to what extent people are Bayesian. 
A follow up analysis assessing  perceived sample size showed participants tended to less sensitive to sample size and associated sampling error for the larger sample size datasets.  

% This may support the sampling hypothesis that people hold only a few samples to represent uncertainty internally. For the large sample size dataset, the normative posterior closely resembled with the observed data regardless of priors. In other words, no matter what participants believe beforehand, participants update their posterior to near the observed data as the observed data is collected from the large group of people. 




 
